Performance of the Vipera framework for DSLs on micro-core architectures

Vipera provides a compiler and runtime framework for implementing dynamic Domain-Specific Languages on micro-core architectures. The performance and code size of the generated code is critical on these architectures. In this paper we present the results of our investigations into the efficiency of Vipera in terms of code performance and size.

==> AcceleratingPythonCodes.tex <==
%\section{Accelerating Python codes}\label{sec:relatedwork}
There are a number of technologies for offloading computation to micro-cores, including OpenCL \cite{richie_coprthr_2014}, BSP \cite{buurlage_bulk-synchronous_2017}, OpenMP \cite{traff_targeting_2015} and MPI \cite{ross_parallel_2015} on the Adapteva Parallella. However, not all are fully implemented, for example OpenMP and MPI. Furthermore, whilst these C-based technologies provide insight into the mechanics of kernel offloading and communications, vPython already provides these capabilities. Therefore, the focus of the investigations presented here are techniques to increase the performance of dynamic programming languages. 

%There are a number of other approaches to accelerating dynamic languages, such as Numba\cite{lam_numba_2015}, Cython\cite{behnel_cython_2011}, ALPyNA \cite{jacob_python_2019}, Copperhead \cite{catanzaro_copperhead_2011}, Parakeet \cite{rubinsteyn_parakeet_2012} and Pallene / Titan \cite{gualandi_pallene_2018}. 
%%\subsection{Related work}
The Python programming language is, at the time of writing this thesis, the most popular programming language\cite{tiobe}. Whilst Python is very popular with programmers, its use of an interpreter results in performance significantly slower than statically compiled languages, such as C\cite{ionescu_investigating_2020} and Fortran\cite{bysiek_migrating_2016}. This has driven the need to overcome the performance overhead of the interpreter and the restrictions imposed by the global interpreter lock (GIL), which effectively makes all Python codes single-threaded by preventing multiple threads from executing Python bytecode at the same time\cite{beazley_understanding_2010}. This has resulted in technologies to increase the performance of existing, single-threaded Python codes through the compilation to native code, including Cython\cite{behnel_cython_2011} and MicroPython\cite{noauthor_micropython_nodate}. The GIL limitation on multi-threading, coupled with the high-throughput parallel processing of GPUs, has resulted in work to leverage GPUs from within Python, including Numba\cite{lam_numba_2015}, Copperhead\cite{catanzaro_copperhead_2011}, Parakeet\cite{rubinsteyn_parakeet_2012}, ALPyNA\cite{jacob_python_2019} and PyCUDA\cite{noauthor_pycuda_nodate}. However, unlike Numba, Copperhead, Parakeet and ALPyNA, PyCUDA does not abstract the generation of GPU code but instead embeds CUDA C code directly within the Python source code. Therefore, it is more related to C-based technologies, rather than the approaches taken by the other technologies to accelerate Python-like codes on GPUs (and CPUs).%, providing little to the discussion of Python code generation techniques and technologies.

The high-level approach of Numba, Copperhead and Parakeet is similar, whereby they define an embedded domain specific language (eDSL) and utilise Python \emph{function decorators} (directives) to annotate the code to be compiled to native code or offloaded to GPUs. %These eDSLs are subset of the Python language to support their code generation techniques. 
For example, Copperhead uses the \texttt{@cu} decorator to mark Copperhead language functions, Parakeet uses the \texttt{@PAR} decorator and Numba defines the \texttt{@jit} decorator to target CPUs, and the  \texttt{@cuda.jit} decorator to target GPUs and perform the necessary data transfer. Listing \ref{lst:numbaexample} is an example of the Numba \texttt{@jit} decorator to generate native code for the \texttt{go\_fast} function. Here, we can also see the impact of the JIT compilation time on the overall execution time, as shown by the two separate timing loops. The  \texttt{nopython=True} parameter of the  \texttt{@jit} decorator, hints to the Numba compiler that the function code can be executed outside the standard Python interpreter, thereby increasing performance. Whilst Numba's JIT compiler can speed up codes by a factor of around 20 times that of the standard Python interpreter \cite{seif_heres_2019}, the generated code is larger than the memory available on micro-core architectures, necessitating a different approach for resource-constrained devices.

Although Copperhead uses a similar decorator approach to Numba, the eDSL uses function primitives to provide data-parallelism for single-dimensional arrays (vectors) of data. The primitives include \texttt{map()}, \texttt{reduce()}, \texttt{gather()}, \texttt{scatter()}, \texttt{replicate()}, \texttt{zip()}, \texttt{permute()} and \texttt{scan()} \cite{catanzaro_copperhead_2011}. Parakeet also employs function primitives to provide data-parallelism on arrays, with codes in both languages appearing very similar, as shown by Listings \ref{lst:copperhead} and \ref{lst:parakeet}.  

\begin{minipage}{0.95\linewidth}
\vspace{\baselineskip}
\begin{lstlisting}[style=pystyle, caption={Numba JIT example \cite{numba_example_nodate}}, label={lst:numbaexample}]
from numba import jit
import numpy as np
import time

x = np.arange(100).reshape(10, 10)

@jit(nopython=True)
def go_fast(a): # Function is compiled and runs in machine code
    trace = 0.0
    for i in range(a.shape[0]):
        trace += np.tanh(a[i, i])
    return a + trace

# DO NOT REPORT THIS... COMPILATION TIME IS INCLUDED IN THE EXECUTION TIME!
start = time.time()
go_fast(x)
end = time.time()
print("Elapsed (with compilation) = %s" % (end - start))

# NOW THE FUNCTION IS COMPILED, RE-TIME IT EXECUTING FROM CACHE
start = time.time()
go_fast(x)
end = time.time()
print("Elapsed (after compilation) = %s" % (end - start))
\end{lstlisting}
\end{minipage}

Copperhead uses CodePy\cite{noauthor_codepy_nodate} to generate OpenMP C code for CPUs and PyCUDA to generate CUDA code for GPUs, achieving 45 to 100\% of the performance of hand-coded CUDA code\cite{catanzaro_copperhead_2011}. Parakeet, like Numba, uses LLVM\cite{noauthor_llvm_nodate} to generate code for CPUs and generates CUDA parallel thread execution (PTX)\cite{noauthor_parallel_nodate} code for GPUs, returning performance 2.4 times slower to 76\% of that of hand-coded CUDA, where the majority of the overhead is due to PTX compilation\cite{rubinsteyn_parakeet_2012}. Both technologies allow Python programmers to leverage GPUs to accelerate their codes without needing to understand the complex programming mechanics of CUDA and embed the accelerated code within their standard Python codes, providing greater accessibility and productivity than using alternatives such as PyCUDA.

\begin{minipage}{0.95\linewidth}
\vspace{\baselineskip}
%procedure for computing $Ax$ for a matrix $A$ in CSR form and a dense vector $x$
\begin{lstlisting}[style=pystyle, caption={Copperhead example \cite{catanzaro_copperhead_2011}}, label={lst:copperhead}]
@cu 
def spmv_csr(vals, cols, x): 
  def spvv(Ai, j): 
    z = gather(x, j) 
    return sum(map(lambda Aij, xj: Aij*xj, Ai, z)) 
    
  return map(spvv, vals, cols)
\end{lstlisting}
\end{minipage}

\begin{minipage}{0.95\linewidth}
\vspace{\baselineskip}
\begin{lstlisting}[style=pystyle, caption={Parakeet example \cite{rubinsteyn_parakeet_2012}}, label={lst:parakeet}]
def add(x,y): 
  return x + y 

def sum(x): 
  return parakeet.reduce(add, x) 

@PAR 
def norm(x): 
   return math.sqrt(sum(x*x))
\end{lstlisting}
\end{minipage}


ALPyNA adopts a different technique to generating GPU code than the eDSL and function decorator approach of Numba, Copperhead, Parakeet. Rather than requiring the programmer to select and annotate the Python functions that will be generated as GPU kernels, ALPyNA analyses loop data dependencies and performs automatic loop parallelisation to generate CUDA kernels for GPUs. ALPyNA leverages the constrained execution flow of Python loops, provided by iterator guarantee of the \texttt{range()} function and lack of a jump (\emph{goto}) construct, to enable the static and dynamic analysis for auto-parallelisation\cite{jacob_python_2019}. ALPyNA only targets GPUs, using the LLVM-based Numba to generate the code. As Listing \ref{lst:alpyna} shows, ALPyNA supports nested loop parallelisation and does not require hints or annotations, making it trivial for the Python programmer to take advantage of the performance increase of up to 1000 times that of the standard Python interpreter (CPython)\cite{jacob_python_2019}. 

\begin{minipage}{0.95\linewidth}
\vspace{\baselineskip}
%n{\"a}ive matrix multiply 
\begin{lstlisting}[style=pystyle, caption={ALPyNA example \cite{jacob_python_2019}}, label={lst:alpyna}]
def matmul(mat_a, mat_b, mat_c): 
  ma_rmax, ma_cmax = np.shape(mat_a) 
  b_rmax, mb_cmax = np.shape(mat_b) 
  for k in range(ma_cmax): 
    for i in range(ma_rmax): 
      for j in range(mb_cmax): 
        mat_c[i][j] = mat_c[i][j] + mat_a[i][k] * mat_b[k][j]
\end{lstlisting}
\end{minipage}


Whilst Numba, Copperhead, Parakeet and ALPyNA provide compelling examples of code generation technologies for CPUs and GPUs, they integrate with the CPython interpreter, restricting their use to traditional desktop\footnote{Here, the definition of desktop is any computer, irrespective of the processor or RAM, running an end-user operating system, such as Linux, Windows or macOS.} and HPC systems, rather than extremely memory-constrained \emph{bare metal} embedded, IoT and micro-core devices. MicroPython\cite{noauthor_micropython_github_nodate}, a version of Python for embedded devices, implements native code generation on embedded CPUs via two \emph{emitters}, \emph{native} and \emph{viper} \cite{george_update_4}, defining the \texttt{@micropython.native} and \texttt{@micropython.viper} decorators to select the emitter for native code generation. The \emph{native} emitter lowers the MicroPython bytecode to machine code and performs calls to VM functions for operations such as arithmetic calculations, binary operations and comparisons. Effectively, this method removes the overhead of the VM's dispatch loop, whilst leveraging the existing VM functions and capabilities. The \emph{viper} emitter takes this approach further by also generating machine code instructions for operations, rather than calling the VM functions. As expected, this increases performance yet further as arithmetic operations are performed inline rather than via a procedure call. This results in performance approximately 10 times that of the \emph{native} emitter and around 24 times faster than the VM interpreter\cite{george_update_5}. The MicroPython cross-compiler can also use the emitters to generate native code on the host, instead of on the device by the standard compiler. It should be noted that the emitters on the device are not JIT compilers as the native code is generated before execution begins and the bytecode is not profiled to select compilation candidates. For MicroPython's embedded targets, the latter approach allows a single MicroPython code file to be deployed to devices with different CPUs (e.g. ARM and Xtensa) where it is then compiled to the specific machine code of the CPU before execution, providing functionality similar to that provided by Java bytecode and the associated JIT compiler within the VM. Whilst MicroPython is specifically designed to target embedded devices, this approach precludes targeting micro-core architectures as it requires 256KB code memory for the VM and compiler, as well as a minimum of 8KB of RAM for the stack and heap\cite{noauthor_micropython_faq_nodate}.

==> OlympusAbstractMachine.tex <==

\section{Olympus native code abstract machine}
\subsection{Overview}\label{sec:ast}
The Olympus abstract machine was designed to meet the requirements for the AOT compilation of dynamic languages, such as vPython. The Olympus approach describes a high-level abstract machine in C that supports dynamic programming languages and provides a simple target for the source language (vPython) compiler. This approach of generating C code, with associated abstract machine \emph{mnemonics}\footnote{Macros or functions that represent abstract machine instructions e.g. \texttt{DECLR} to declare a real object, \texttt{STI} to store an integer, \texttt{ADDRL} to address a local object and \texttt{MKLAMBDA} to create the structure containing a lambda and its static environment.}, is described in \cite{jamieson_compact_2021}.
%informed by the Anubis\footnote{Anubis\cite{gibbs_jamieson_tindale_1991} is a persistent\cite{dearle_orthogonal_2010} Object-Oriented \ programming language that contains powerful programming abstractions, such as \emph{first-class procedures}\cite{atkinson_persistent_1984} and \emph{anonymous functions} (lambdas)\cite{ranta_implementing_2012}, with their respective closure support.} abstract machine and is similar to the cross-platform, macro-based, code generation approach used by \cite{koch_algol68_1975}. However, the Olympus abstract machine addressing model, based on that for Merlin, is static and generated by the compiler, whereas the Anubis abstract machine performs dynamic chaining through the environment to lookup objects, in a similar manner to the searching of the symbol table in the ePython virtual machine. 
However, the Olympus abstract machine was updated for vPython and separates object addressing from the operation mnemonics, enabling the support for all areas of micro-core memory hierarchies and the placement of objects on the stack or in the heap, as required. The mnemonic model allows code generation complexity to be managed in the compiler or abstract machine, as is expedient. For example, the instructions required to copy a function return value before the stack frame is \emph{retracted} could be generated individually by the source language compiler or they could be implemented as steps within the function \texttt{APPLY} and \texttt{RET} mnemonics. Moreover, if the complexity is hidden within the abstract machine mnemonics, the code generation routines within the compiler do not need to be changed if the decision is made at a later date to manage source function return values using C's in-built function call mechanisms. %Currently, the mnemonic model allows Olympus to manage cross-compiler issues. For example, the different function call order of GCC and Clang is managed by the \texttt{EXPR} mnemonic that performs no operation for GCC but stacks the return values of expression mnemonics containing multiple function calls to ensure the correct evaluation order for Clang. The Olympus code generator does not need to be aware of the C compiler being used to compile the generated abstract machine mnemonics, it only has to emit a wrapping \texttt{EXPR} mnemonic for expressions containing multiple function calls. 


\subsection{Type management}
All target object declarations are typed, either via type inference performed on the AST for the vast majority of codes or directly from type annotations\footnote{In the case of ePython, these are the type constructor functions \texttt{int()}, \texttt{float()} and \texttt{str()} which can be considered similar to the casting operators in C, and can be used to help the compiler infer types when it returns an error that it is unable to do so.} in the source code. Furthermore, all object access is similarly typed, with dynamic changes of an object type resulting in a new typed declaration and updated typed access from that point of execution onward. This is managed by creating a new \texttt{ASTdeclaration} and associated \texttt{ASTidentifier} node within the AST with the updated type. It is important to note that this does not require the abstract machine to allocate any additional space within the stack frame for the new object as, by default, \emph{compound types} (arrays and complex numbers) are allocated in the heap, with a reference to the new object replacing the previous value stored within the frame. This model removes the requirement to perform dynamic runtime type checking and this approach to typing is similar to the simple type freezing performed by \cite{cheng_type_2020} in that runtime type checks are not performed on objects, thereby eliminating the associated overhead and increasing performance. %% Whilst this might appear to restrict dynamic typing somewhat, taking the \emph{Awesome Python} list of applications \cite{chen_vintaawesome-python_2020}, approximately 80\% of the identifiers in the code do not have a dynamic type, and as such it was concluded it is reasonable to restrict the use of this feature. 

\subsection{Memory access and operation mnemonics}\label{sec:framemanagement}
Listing \ref{lst:access} is an example of the typed object access in the generated Olympus abstract machine C code. % for the memory layout visualised in Figure \ref{fig:frames}. 
In this example, the real part of the \texttt{complex} object at the enclosing (\emph{foreign}) scope level 1 and offset 2 (\texttt{ADDRF(1,2)}) is being set to the value \texttt{4.3} by the store complex real (\texttt{STCR}) mnemonic. The second line updates the integer element indexed by the object at offset 0 (\texttt{LDI(ADDRL(0))}) of a vector stored in the heap and declared in the local scope at offset 1 (\texttt{ADDRL(1)}), the value \texttt{42} .

\begin{minipage}{0.95\linewidth}
\vspace{\baselineskip}
\begin{lstlisting}[style=cstyle, caption={Object access example}, label={lst:access}]
STCR(ADDRF(1,2),4.3);
STAI(ADDRL(1),LDI(ADDRL(0)),42);
STR(ADDRF(4,1),10.0);
\end{lstlisting}
\end{minipage}

%Figure \ref{fig:frames} also highlights that 
The scope level increases outwards from the local block (or function) scope, with local objects having a scope level of zero. This enables the C compiler to use indexed addressing from the frame pointer to access local objects, thereby increasing performance for local objects and loop block indices, as the compiler can use indexed addressing to directly access the local objects.  Furthermore, the indexing of outer scope levels directly removes the need to chain up environment frames to locate non-local objects, with the corresponding performance overhead. This model also allows support of Python 3 \texttt{nonlocal} objects \cite{noauthor_7_2020} that are declared in the nearest enclosed scope level. 

%In the Olympus abstract machine C code, the object access APIs are implemented as mnemonics that directly update the frame elements within the environment and include the required casting to and from the current object type, as shown at line 3 of Listing \ref{lst:access}.%, where the \texttt{STR} and \texttt{ADDRF} mnemonics combined expand to \texttt{((*(Real*)(\&((Value*) memory$\rightarrow$senv[(level)])[(offset)])) = (Real)(value))}. These not only access the frame element directly, but also ensure that the value is stored correctly in memory. As in this example, casting a real value to and from the generic \texttt{Value} field within the static environment (\texttt{memory$\rightarrow$senv}). Whilst, conceptually, Olympus utilises an environment link described by \cite{bornat_understanding_2020}, the implementation is different. The approach here is to store the current display frame (\texttt{memory$\rightarrow$frame}) as the \textlambda{}'s static environment within the \texttt{Lambda} structure created by the \texttt{MKLAMBDA} mnemonic at the time of declaration. This allows the Olympus abstract machine to support first-class and nested functions. 

%The variable referencing mnemonics of the initial Olympus memory referencing model, described in \cite{jamieson_compact_2021}, coupled the addressing of objects within the frames to the operation. However, in order to support multiple levels in the memory hierarchy and compound types such as complex numbers on the stack, as well as in the heap, the separation of addressing from operation within the mnemonics was required. 
The separation of object addressing from operation within the mnemonics, introduced for vPython, simplified the implementation of object references (the \texttt{\&} operator in vPython and the \texttt{id()} function in Python) within the abstract machine as the \texttt{ADDRL} and \texttt{ADDRF} mnemonics can provide the object address within the stack or the heap. The implementation of object references %and the unified \texttt{Memory} structure discussed in Section \ref{sec:functionmodel}, 
enables the integration of Olympus applications with C frameworks, such as the Eithne benchmarking framework\cite{noauthor_maurice_nodate} and MPI (Message Passing Interface)\cite{openmp}.


==> vPythonCompiler.tex <==
\subsection{vPython}\label{vpython}
vPython is a development of the ePython programming language, originally developed for teaching parallel programming on the Epiphany-III micro-core architecture\cite{brown_epython_2016} and later developed into an embedded Domain-Specific Language (eDSL) within Python\footnote{The ePython eDSL can be embedded within any Python environment running on the host.} running on the host to enable the offloading of kernels to micro-core accelerators\cite{brown_offloading_2017}. Here, specific functions can be annotated as kernels for offloading to the micro-cores and there are a set of communication functions that allow the programmer to control the transfer of data to and from the host\cite{brown_offloading_nodate}. For example, Listing \ref{lst:epython_offload} illustrates how the \texttt{@offload} function decorator can be used to mark the \texttt{helloworld()} function for download to the micro-cores for execution. This example also shows the implicit transfer of data to and from the micro-cores; the values of the input parameters \texttt{a=10} and \texttt{b=20}, and the return value (a list of the value \texttt{30}, one value for each core in the micro-core accelerator. %\footnote{In the case of a single Adapteva Epiphany-III processor, a list of 16 elements of the value \texttt{30(a+b}$\Rightarrow$\texttt{10+20)} is returned i.e.\texttt{[30,30,30,30,30,30,30,30,30,30,30,30,30,30,30,30]} }). 

As part of the parallel programming support, vPython provides core-to-core and host-to-core communications via the \texttt{send()} and \texttt{recv()} functions, as well as \emph{collective communications} via the \texttt{reduce()} function call with the operations \texttt{max}, \texttt{min}, \texttt{sum} and \texttt{prod}. The \texttt{bcast()} function is provided to broadcast a value from one core to all the other cores\cite{brown_epython_2016}. With these functions, vPython programmers are able to create parallel codes that leverage the multiple cores of the micro-core processor.

\vspace{\baselineskip}
\begin{lstlisting}[style=pystyle, caption={Synchronous kernel launch example\cite{brown_offloading_nodate}}, label={lst:epython_offload}]
from epython import offload

@offload
def helloworld(a,b):
  print "Hello World"
  return a+b

print helloworld(10, 20)
\end{lstlisting}

\section{vPython compiler}\label{vpythoncompiler}
Figure \ref{fig:astflow} shows the Olympus code generation phases for a dynamic language such as vPython. The compiler phases are \emph{pipelined}, where the module to generate the AST in Phase 1 is separate from the phases that perform \emph{type inferencing}, optimisation and the generation of the Olympus abstract machine code, with the output of one phase (the AST) being \emph{piped} into another. The vPython lexer and parser are written using Flex and Bison, respectively. As the output of Phase 1 is an AST, parsers for other languages could be written using alternative technologies, or using a manually written recursive descent parser, as long as they generate an Olympus-compatible AST. Furthermore, as the Olympus compiler phases can be pipelined via a textual representation of the AST, a new compiler does not need to be written in a C-based technology.
%\footnote{The production version of the ePython compiler performs the different phase operations on the in-memory AST, rather than using files / pipes between the individual phases.} 

%This also allows the AST to be dumped as a textual representation, or to generate a graph using Graphviz \cite{noauthor_graphviz_nodate}. The textual AST files enabled the testing of individual AST processing phases 2-4 (type inference, basic optimisation and code generation), without having to run the code end-to-end. A downside of this approach was the impact to both the AST writing / parsing code when structural changes were made to the AST, increasing development effort. However, this was offset by the reduction in the time taken to fault-find code generation issues, as they could be isolated phase by phase where the textual representation of an AST of previously compiled vPython codes from Phase 1 could be used as the test input for each phase and the visual representation (Graphviz) of the output AST inspected. 



\begin{figure}[h!]
\centering
%%\includegraphics[height=10em]{images/ELF.png}
\includegraphics[width=0.95\textwidth]{images/Codegen_flowchart_v1d1.pdf}
\caption{Olympus code generation phases}
\label{fig:astflow}
\end{figure}

As shown in Figure \ref{fig:astflow}, the code generation phase (Phase 4) can support different \emph{pluggable} code generator \emph{targets}, for example, Olympus abstract machine C source code and Merlin\cite{jamieson_merlin} assembly language files (\texttt{.asm}), thereby allowing different target code to be generated from the same AST. Two code generators have currently been fully developed: one for the Olympus C abstract machine and another for the Graphviz \texttt{.dot} file format to allow the structure of the AST to be inspected. %The feasibility of pluggable executable code generators was tested by creating a code generator for a subset of the Merlin assembly language. The key driver for the pluggable code generator target API was to enable the future implementation of a vPython bytecode target to allow the replacement of the existing vPython monolithic bytecode compiler and the future implementation of hybrid Olympus native code / bytecode kernels.

